Testing the universality of the star formation efficiency in dense molecular gas

Recent studies have suggested that star formation (SF) in dense gas may be governed by essentially the same law in Galactic clouds and external galaxies. This conclusion remains controversial, however, because different tracers have been used to probe the dense gas mass in Galactic and extragalactic studies. We conducted observations of Aquila, Oph., and Orion B in HCN(1-0), HCO$^+$(1-0), and their isotopomers to calibrate the HCN and HCO$^+$ lines used as dense gas tracers in extragalactic studies and to test the possible universality of the star formation efficiency in dense gas, SFE$_{dense}$. H$^{13}$CO$^+$ and H$^{13}$CN were observed to be good tracers of the filaments detected with Herschel. Comparing the luminosities $L_{HCN}$ and $L_{HCO^+}$ with the reference masses $M_{Herschel}^{Av>8}$, the empirical conversion factors $\alpha_{Herschel-HCN}$ and $\alpha_{Herschel-HCO^+}$ were found to be anti-correlated with the local FUV strength. In agreement with Pety et al. (2017), HCN and HCO$^+$ were also found to trace gas down to Av>2. As a result, published extragalactic HCN studies must be tracing all of the moderate density gas. Estimating the contribution of this moderate density gas from the typical column density PDFs in nearby clouds, we obtained the following $G_0$-dependent HCN conversion factor for external galaxies:$\alpha_{Herschel-HCN}^{fit'}=64\times G_0^{-0.34}$. Re-estimating the dense gas masses in external galaxies with $\alpha_{Herschel-HCN}^{fit'}$, we found that SFE$_{dense}$ is remarkably constant over 8 orders of magnitude in dense gas mass. Our results confirm that SFE$_{dense}$ of galaxies is quasi-universal on a wide range of scales from ~1-10pc to >10kpc. Based on the tight link between SF and filamentary structure found in Herschel studies of nearby clouds, we argue that SFE$_{dense}$ is primarily set by the microphysics of SF in filaments.

==> Table_int_range.tex <==
\begin{table*}
\centering
\begin{threeparttable}
\caption{Integrated velocity range\label{table:integ_range}}
\begin{tabular}{lccccc}
\hline
Region &  $V_{\rm peak, H^{13}CO^+}$  & HCN (1--0) & HCO$^{+}$ (1--0) & H$^{13}$CO$^+$ (1--0) &  H$^{13}$CN (1--0) \\
            &  [km/s]  & [km/s]  & [km/s]  & [km/s]  & [km/s]   \\
\hline
Aquila  & 7.0 & -8.15 -- 22.08 &  -8.15 -- 22.08   & 3.42 -- 10.52 & -3.03 -- 17.12 \\
Oph     & 3.5 & -6.50 -- 13.56 & -6.50 -- 13.56   & 0.91 -- 6.03   & -6.50 -- 13.56 \\
Orion B/NGC2023 & 10.0 &  -0.05 -- 20.05 & -0.05 -- 20.05 & 7.45 -- 12.55 & -0.05 -- 20.05 \\
Orion B/NGC2024 & 10.9 &  0.85 -- 20.95 & 0.85 -- 20.95 & 7.85 -- 12.95 & 0.85 -- 20.95 \\
Orion B/NGC2068 & 10.9 &  0.85 -- 20.95 &  0.85 -- 20.95 & 7.85 -- 12.95 & 0.85 -- 20.95 \\
Orion B/NGC2071 & 9.5 &  -0.55 -- 19.55 &  -0.55 -- 19.55 & 6.95 -- 12.05 & -0.55 -- 19.55 \\
\hline
\end{tabular}
\end{threeparttable}
\end{table*}


